Non-local Recurrent Neural Memory for Supervised Sequence Modeling

Typical methods for supervised sequence modeling are built upon the recurrent neural networks to capture temporal dependencies. One potential limitation of these methods is that they only model explicitly information interactions between adjacent time steps in a sequence, hence the high-order interactions between nonadjacent time steps are not fully exploited. It greatly limits the capability of modeling the long-range temporal dependencies since one-order interactions cannot be maintained for a long term due to information dilution and gradient vanishing. To tackle this limitation, we propose the Non-local Recurrent Neural Memory (NRNM) for supervised sequence modeling, which performs non-local operations to learn full-order interactions within a sliding temporal block and models global interactions between blocks in a gated recurrent manner. Consequently, our model is able to capture the long-range dependencies. Besides, the latent high-level features contained in high-order interactions can be distilled by our model. We demonstrate the merits of our NRNM on two different tasks: action recognition and sentiment analysis.

==> experiments.tex <==
We validated our model on three public datasets. 
These three data sets belong to three different tasks: (1)Language modeling, 
(2)Sentiment Analysis, and (3)Action recognition, which prove the generalization ability of our model.

Our main goal is to propose a new model to solve the problem of long-range sequence problems, 
so we do not make extreme explorations for a certain task, such as the use of specific structures, parameter searching and tricks.

\subsection{Language Modeling}
A Language model learns the probability of word occurrence given the words that precede it. Language modeling is 
useful in various applications such as speech recognition and meachine translation, and is one of the important issues in natural-language processing.
The language model can be seen as a one-to-sequence problem, and we can evaluate the performance of our model in one-to-sequence mode through this experiment.

\subsubsection{Dataset}
We used the Penn Treebank(PTB) dataset\cite{marcus1993building} for word-level Language modeling. It is a widely used and highly studied benchmark 
for language modeling. PTB dataset contains 888k training words, 70k validation words and 79k testing words. It has 10K words in its vocabulary. 

\begin{table}[!htbp]
    \centering
    \caption{Penn TreeBank(word level)Dataset}
    \begin{tabular}{cccc} 
    \toprule
     & Train & Val & Test \\  
    \midrule       
      Tokens   & 888K  & 70K & 79K\\
      Vocab size  & \multicolumn{3}{c}{10K} \\
    \bottomrule
    \end{tabular}
\end{table}
 
\subsubsection{Experimental Setup}
There are some works dedicated to the language modeling task that have been explored in terms of regularization\cite{krueger2016zoneout}\cite{zaremba2014recurrent}, dropout\cite{gal2016theoretically} 
and specific structures\cite{grave2016improving} etc.,which has greatly improved this task.

What we mainly need to verify is the performance of our model. In order to ensure the fairness of the test,we follow standard practice and use the the 
Pytorch\footnote{\url{https://github.com/pytorch/pytorch}} official code \footnote{\url{https://github.com/pytorch/examples/tree/master/word_language_model}} to 
implement the experiment. Data processing and testing settings are the same as \cite{krueger2016zoneout}. 
We have adopted the word embedding to 512-dimensional, using 512 hidden units and 2 layers of LSTM, the weights initialized uniformly $[-0.1,+0.1]$. The dropout ratio is 0.5. 
We use the SGD optimizer to train the model with an initial learning rate of 20 and anneal the learning rate with a factor of 0.5 when validation accuracy on plateaus, and gradient norms are clipped at 0.3. 
And we use the cross entropy loss function to optimize the model.

Our NRNM model uses the same training and test hyper parameters as above, while adding three additional parameters: stride($s$), block length($bl$) and memory dimension($m$).
In the experiment, we set $m$ to 512, $s$ to 1 and $bl$ to 4.

We use \textbf{perplexity}($PPL$)\cite{neubig2017neural} to measure the model accuracy. A \textbf{low perplexity} indicates the model is good at predicting the sample. 
$PPL$ can be expressed as the exponent of the average negative log likelihood for each word.
$$PPL(\varepsilon _{test};\theta )=e^{-(log(P(\varepsilon _{test}; \theta ))/length(\varepsilon _{test}))}$$
$\theta$,$\varepsilon _{test}$ and $length(\varepsilon _{test})$ represent the parameters of model, test dataset and the number of words in the corpus respectively.

\subsubsection{Results and Discussion}
\mycomment{need figure and detail}

We didn't do much searching on model structure and parameters, and using more tricks for this task, we have the ability to improve the 
PPL by 4.3, from 78.4 to 74.1.Under the same conditions, we reported the best performance in Table~\ref{PTBresults}. 

Our model's performance have improved with \cite{gal2016theoretically},which is aim to this task, that shows our
our method can be effectively embedded into other frameworks to improve performance.

\begin{table}[htbp]
    \centering
    \caption{PTB results}
    \label{PTBresults}
    \begin{tabular}{ccc}   
    \toprule
     Model & valid(ppl) & test(ppl) \\  
    \midrule       
    Variational(tied,medium)\cite{gal2016theoretically}  & 81.8  & 79.7 \\
    Variational(tied,large)\cite{gal2016theoretically}  & 77.3  & 75.0 \\
    Variational(MC,large)\cite{gal2016theoretically}  &  - & 73.4 \\
    LSTM\cite{grave2016improving}  & -  &82.3 \\
    Neural cache model\cite{grave2016improving}  & -  & 72.1 \\
    LSTM\cite{krueger2016zoneout}  & -  &78.4 \\
    LSTM+zonout\cite{krueger2016zoneout}  & -  &77.4 \\
    Our LSTM(baseline)  & 81.80  & 77.97 \\
    Our NRNM           & 77.58  & 74.35 \\
    Our NRNM+Variational\cite{gal2016theoretically}        & 72.8  & 69.92 \\
    \bottomrule
    \end{tabular}
\end{table}

\subsection{Sentiment Analysis Experiments}
Sentiment analysis is a basic research topic in the field of natural language processing, 
and it is widely used in many practical applications such as social media and reviews. 
The language modeling task can be seen as an one-to-sequence application, and sentiment analysis is a 
sequence-to-one problem. We will use this experiment to further prove the robustness of our model.

\subsubsection{Dataset}
We used the IMDB dataset which is a movie review dataset provided by \cite{maas2011learning} to evaluate our model.

IMDB is a stardard benchmark for sentiment analysis. It contains 50000 labeled which is divided into 25000 training samples 
and 25000 testing samples and 50000 unlabeled reviews form IMDB. The average sample length is 241 words and the max length is 2526 words\cite{dai2015semi}. 
This task mainly consists of two categories: positive and negative.
It is worth noting that this task is often used for semi-supervised learning\cite{dai2015semi}\cite{johnson2016supervised}\cite{miyato2016adversarial} 
and others\cite{dieng2016topicrnn}\cite{radford2017learning}, and that 50k unlabeled data is used. However, in this work, only labeled data is used.

\subsubsection{Experimental Setup}
We also did not search for model parameters in this experiment.The torchtext\footnote{\url{https://github.com/pytorch/text}} was used for data preprocessing.
We set word embedding dimension as 300 and we utilize 300-dimensional Glove word vectors pretrained by \cite{pennington2014glove}. We use 3 layer of LSTM, 
the hidden size is 512 and the dropout rate of embedding layer is set to 0.5. According to the experimental method used in \cite{dai2015semi}, we also experimented 
pre-train a language model fro roughtly 100 epoch , and then we use the weight of embedding layer parameters to initialize the LSTM for training the classifier.

We train our model by Adam\cite{kingma2014adam} optimizer with the initial learning rate is 0.0001. The weigth decay is set to $1e-5$.
And pre-train the Language model by SGD optimizer, which the initial earning rate is 20.
The loss function for sentiment classification is a binary cross-entropy function. 

This is a classification problem, and we use the accuracy to measure the performance of the model.

\subsubsection{Results and Discussion}

For baseline LSTM, we reproduced the same accuracy with Glove word vectors.
Using the same experimental conditions as baseline LSTM, our NRNM increased the accuracy by 1.61\%.
When we adopted the training method in \cite{dai2015semi}(show as NRNM* in the Table~\ref{IMDBresults}) we achieved 93.11\%.
With labeled data only, we achieved the best results.

This experiment proves that our model is also very robust to the task of this text classification, 
or it is also effective for sequence-to-one problems.

\begin{table}[!htbp]
    \centering
    \caption{IMDB result in accuracy(\%)}
    \label{IMDBresults}
    \begin{tabular}{cc}   
    \toprule
     & Accuracy  \\  
    \midrule    
    LSTM\cite{xia2018model}  & 89.9\% \\
    MLDL\cite{xia2018model}  & 92.59\% \\
    GLoMo\cite{yang2018glomo}  & 89.16\% \\
    LM-LSTM\cite{dai2015semi}  & 92.36\% \\
    SA-LSTM\cite{dai2015semi}  & 92.76\% \\
    oh-2LSTMp\cite{johnson2016supervised}  & 91.86\% \\
    BCN+Char+CoVe\cite{mccann2017learned}  & 92.1\% \\
    Virtual\cite{miyato2016adversarial}   & 94.1\% \\
    LSTM(baseline)   & 89.46\%  \\
    NRNM            & 91.07\%   \\
    NRNM*           & 93.11\%   \\
    \bottomrule
    \end{tabular}
\end{table}

\subsection{Action Recognition Experiments}

Human action recognition is an important branch of computer vision research. 
It is widely used in video surveillance, human-computer interaction, video understanding and 
so on\cite{poppe2010survey}\cite{weinland2011survey}\cite{aggarwal2011human}.

Action recognition is divided into two categories: RGB video-based and 3D skeleton-based methods.
The video-based methods focus on spatial information on single-frame RGB images and temporal informationon the video stream.
The skeleton-based methods, which can effectively shield environmental factors such as illumination changes and background changes by extracted 
the 3D coordinate position of human keypoint, so that more attention has been paid in recent years.

There are lots of work\cite{du2015hierarchical}\cite{shahroudy2016ntu}\cite{wang2017modeling}\cite{lee2017ensemble}\cite{zhang2017view}\cite{song2018spatio}
applied recurrent neural networks on the action recognition, because of RNN has strong sequence data learning capabilities.
They have made a lot of efforts on this task from the aspects of temporal-spatial relationship, connection of key points of the human body, network structure and so on.

\subsubsection{Dataset}
We use the NTU dataset\cite{shahroudy2016ntu}, which is currently the largest action recoginition dataset.
It contains 56,880 video sequences, about 4 million frames, and is divided into 60 action categories.
The person in each frame use Microsoft Kinect to extract 3D coordinate points of 25 body joints.
According to \cite{shahroudy2016ntu}, there are two kinds of evaluation matrixs: Cross-Subject(CS) and Cross-View(CV).
For the CS setting, 40 subjects were equally divided into training sets and test sets. For the CV settings, 
the videos acquired by the first two cameras is used for training and the rest is used for testing.
We will evaluate the performance of our model in these two metrics.

\subsubsection{Experimental Setup}
The input to our network is a 150-dimensional vector, including the 3-D coordinate of 25 body joints for 2 people (if there is only one person, copy this person again).
We refer to the settings of \cite{tu2018spatial}, we also use Zoneout\cite{krueger2016zoneout} to regularize the network.
We use 3 layers of LSTM as baseline, each layer containing 128 hidden units.Our NRNM also uses 3 layers and uses 128-dimensional memory cells.We also have 
the Memory cell of 256-D and 512-D, which will be analyzed in detail later. We use a dropout of 0.5 ratio to prevent overfitting.
The optimizer is Adam\cite{kingma2014adam}, and the initial learning rate is 0.001.

We use cross-entropy as the loss function and use accuracy to evaluate the performance of the model.


\subsubsection{Results and Discussion}

\textbf{Evaluation of Model Performance.}
In the following experiments, we are all implicit to learn the relationship between the body joints in single-frame and the temporal correlation between 
different time steps directly, rather than explicitly adjusting any additional information, such as joint connection, human body structure modeling and so on.

The results of our work and other models are compared in Table~\ref{NTUresult}. 
Under the CS settings, we increased by 10.5\% and 2.7\% , respectively, over the baseline LSTM model and Zoneout LSTM model.
In addition, under the CV setting, we have improved 9.4\% and 3.3\% respectively than the baseline LSTM model and the Zoneout LSTM model.
Under certain conditions, we are better than all current LSTM-based methods, and we have achieved comparable results with other current algorithms.

\begin{table}[!htbp]
    \centering
    \caption{NTU-RGBD result in accuracy(\%)}
    \label{NTUresult}
    \begin{tabular}{ccc}   
    \toprule
     & CS & CV  \\  
    \midrule        %画一条横线
    HBRNN-L\cite{du2015hierarchical}  & 59.1 & 64.0 \\
    Part-aware LSTM\cite{shahroudy2016ntu} & 62.9 & 70.3 \\
    Trust Gate ST-LSTM\cite{liu2016spatio} & 69.2 & 77.7 \\
    Two-stream RNN\cite{wang2017modeling} & 71.3 & 79.5 \\
    Ensemble TS-LSTM\cite{lee2017ensemble} & 74.6 & 81.3 \\
    VA-LSTM\cite{zhang2017view} & 79.4 & 87.6 \\
    STA-LSTM\cite{song2018spatio}   & 73.4 & 81.2 \\
    EleAtt-LSTM\cite{zhang2018adding} & 78.4 & 85.0 \\
    EleAtt-GRU\cite{zhang2018adding} & 79.8 & 87.1 \\
    EleAtt-GRU(aug.)\cite{zhang2018adding} & 80.70 & 88.4 \\
    LSTM(baseline)   & 70.31 & 79.64 \\
    LSTM+zonout      & 78.14 & 85.73 \\
    NRNM(ours)        & 80.80 & 89.00 \\
    \bottomrule
    \end{tabular}
\end{table}

\textbf{Evaluation of Long-Range Modeling.}

\mycomment{Different lengths of block size have different results.}

In order to demonstrate the ability of our long range  temporal modeling, we use different sliding 
window sizes($win$) to evaluate the accuracy of the model when other hypermeters are fixed.

Under the CV setting, we take the sliding windows($win$) as 0, 4, 6, 8, 10, and 12, respectively, which 0 means baseline model. 
From the experimental curve, Figures~\ref{fig:CV_slide}, it can be explored that the accuracy increases as the $win$ 
increases until it reaches a saturated state and then falls.This is a good illustration of the ability of our model to 
extract information over long range temporal.
\begin{figure}[t]
\begin{center}
\includegraphics[width=0.4\textwidth]{images/CV_slide.jpg}
\end{center}
\caption{ablation 1}
\label{fig:CV_slide}
\end{figure}

\textbf{Evaluation of Variational Model Architecture.}
The location of the memory insertion also has a large impact on the model, and different 
adjustments may be required for different tasks. 
In order to get this rules, we added the NRNM unit in different layers, and the results are 
shown in Figures~\ref{fig:memory_location}. From this experiment, we can find that it is not necessary 
to add a NRNM unit to each layer. Adding a NRNM unit on each layer alone can have a better improvement effect, 
but using memory across layers is not a good way. 
Using NRMN unit close to the input layer can get better results, which also shows that we have better 
extraction ability for low-level semantic features.
We recommend adding NRNM unit in the input layer and the hidden layer. For example, if we use 3 layers of lstm for our task, 
we will add NRMN units at layer 0 and layer 1.

Inspired by the overlapping sampling of the convolution kernel in the CNN when sampling features, 
we also support adjustable update of the memory in NRNM unit, rather than limited to the block lenght of LSTM.
This adjustable update method is especially important for long range temporal(such as  over 20 time steps), 
because when the sliding window is very large, the information loss is very serious, and the 
adjustable update memory can complement the information close to the current moment.
For example, when we take 20 as the length of the sliding window, and we take hidden of LSTM every 10 time steps.
If we update the memory only once for each block, then every time we get the memory is the information before 20 time steps, 
the timeliness of the information is lost. By adjustable update we can updated every 10 time steps, which is a good way to 
ease this problem.The relevant experimental results are shown in Table~\ref{table:dinamic_update}.
By changing the update step size, the performance is improved for long range temporal,which is 20 in the experiment.

In addition, we also explored the impact of depth and memory size of NRNM, the results are shown in 
Table~\ref{table:deepth} and ~\ref{table:m_size}.\mycomment{Need more details....}

\begin{figure}[t]
\begin{center}
\includegraphics[width=0.4\textwidth]{images/memory_location.jpg}
\end{center}
\caption{ablation 1}
\label{fig:memory_location}
\end{figure}

\begin{comment}
\begin{table}[!htbp]
    \centering
    \caption{NTU-RGBD Ablation study 2(about memory insertion location(128-dim))(\%)}
    \label{table:memory_location}
    \begin{tabular}{ccc}   
    \toprule
     & CS  \\  
    \midrule      
    s5b10mix0  & 79.03  \\
    s5b10mix1  & 79.66  \\
    s5b10mix2  & 79.13  \\
    s5b10mix01  & 79.27  \\
    s5b10mix02  & 78.52 \\
    s5b10mix12  & 78.68 \\
    s5b10mix012  & 78.94 \\
    \bottomrule
    \end{tabular}
\end{table}
\end{comment}

\begin{figure}[t]
\begin{center}
\includegraphics[width=0.4\textwidth]{images/sliding_windows.jpg}
\end{center}
\caption{sliding windows}
\label{fig:sliding_windows}
\end{figure}

\begin{table}[!htbp]
    \centering
    \caption{NTU-RGBD Ablation study 5(about deepth (256-dim, mixm01))(\%)}
    \label{table:deepth}
    \begin{tabular}{ccc}   
    \toprule
     & CS\\  
    \midrule  
    s5b10-1layer  & 76.69 \\
    s5b10-2layer  & 77.91 \\
    s5b10-3layer  & 79.49 \\
    s5b10-4layer  & 79.47 \\
    \bottomrule
    \end{tabular}
\end{table}

\begin{table}[!htbp]
    \centering
    \caption{NTU-RGBD Ablation study 6(about memory size)(\%)}
    \label{table:m_size}
    \begin{tabular}{ccc}   
    \toprule
     & CS \\  
    \midrule  
    s4b8mixm012-128  & 78.64 \\
    s4b8mixm012-256  & 79.37\\
    s4b8mixm012-512  & 78.75\\
    \bottomrule
    \end{tabular}
\end{table}

\begin{figure*}[t]
\begin{center}
\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}
\end{center}
   \caption{view of memory weight and action serial}
\label{fig:long}
\label{fig:onecol}
\end{figure*}
